"In-Context Learning" or: How I learned to stop worrying and love "Applied Information Retrieval"

With the increasing ability of large language models (LLMs), in-context learning (ICL) has evolved as a new paradigm for natural language processing (NLP), where instead of fine-tuning the parameters of an LLM specific to a downstream task with labeled examples, a small number of such examples is appended to a prompt instruction for controlling the decoder's generation process. ICL, thus, is conceptually similar to a non-parametric approach, such as $k$-NN, where the prediction for each instance essentially depends on the local topology, i.e., on a localised set of similar instances and their labels (called few-shot examples). This suggests that a test instance in ICL is analogous to a query in IR, and similar examples in ICL retrieved from a training set relate to a set of documents retrieved from a collection in IR. While standard unsupervised ranking models can be used to retrieve these few-shot examples from a training set, the effectiveness of the examples can potentially be improved by re-defining the notion of relevance specific to its utility for the downstream task, i.e., considering an example to be relevant if including it in the prompt instruction leads to a correct prediction. With this task-specific notion of relevance, it is possible to train a supervised ranking model (e.g., a bi-encoder or cross-encoder), which potentially learns to optimally select the few-shot examples. We believe that the recent advances in neural rankers can potentially find a use case for this task of optimally choosing examples for more effective downstream ICL predictions.

==> wps.tex <==
\subsection{Proposed Work packages}

We propose to structure the project into four different work packages, each with its own set of research questions.

\uls
\li \textbf{WP-1}: The first work-package will be based on \textbf{misinformation detection} of LLMs. It is a widely known fact that the text generated by LLMs are often of hallucinatory in nature \cite{dziri-etal-2022-origin,10.1145/3571730}. Consequently, mapping back to the original documents (attribution at document level \cite{bohnet2023attributed}) which were likely responsible in affecting the decoding path to generate the text for a downstream task can throw insights on an LLM's 0-shot or few-shot (in-context) task-specific abstraction of the input data.


\li \textbf{WP-2}: In the second work-package, we will investigate
\textbf{Prompt or In-Context Explanations} of the LLM-generated content in terms of attention-based or counter-factual explanations of the prompts, i.e., which parts of the prompts are more important in determining the class probabilities (via generation of class-specific sets of words by the decoder).

\li \textbf{WP-3}: In this work package, we will seek towards achieving \textbf{fair predictions} with ICL. More specifically, when data instances are associated with sensitive attributes, such as demographics etc., we aim to reduce ICL-based predictions that are stereotypical in nature, e.g., not predicting frequently that colored people are more prone to recidivism \cite{propublica,adDelivery}.  

\li \textbf{WP-4}: The fourth work-package will put together all the research components of the above mentioned work packages towards constructing an effective ICL-based predictive model for a downstream task, and will \textbf{evaluate the overall system performance}. More concretely speaking, in addition to the overall effectiveness (e.g., precision, recall) we will also measure the explainability (fidelity of explanations), fairness and user trust (in terms of controlled user studies).


\ule


\section{Approach}  \label{sec:approach}

In this section, we outline the approaches to be undertaken towards answering the research questions outlined in the four work packages.

\subsection{WP-1: Misinformation Detection}

Given an LLM-generated content, we propose to address the following three different tasks with increasing levels of complexity.
\ols
\li \textbf{Binary misinformation classification}: Does a piece of text contain false information?
\li \textbf{Fine-grained misinformation classification}: If a text segment constitutes of misinformation, what type of misinformation it is, e.g., inaccurate quantities, false attribution etc.
\li \textbf{Extracting or summarising the misinformation}: Identify the part of the text (as a span of words) that constitutes this misinformation.
\ole

\subsubsection{Binary classification}
Detecting if a text segment contains misinformation is a binary classification problem. We plan to investigate standard parametric supervised approaches, such as task-specific fine tuning of transformer architectures, e.g., BERT \cite{devlin2019}. This requires creating labeled data with two class labels.

To construct a relatively large resource of training data, in addition to training our models on existing datasets (e.g. FEVER \cite{thorne2018fact}), we also plan to \textbf{generate simulated text} with the help of large language models (LLMs). More precisely, we plan to use instruction tuned LLMs, such as Llama \cite{llama} or FlanT5 \cite{chung2022scaling} to formulate appropriate prompts guiding the models towards generating misinformation. In fact, we are currently organising a shared task where we released a dataset of prompt-based LLM generated misinformation \cite{ilsum}.   

\subsubsection{Fine-grained misinformation classification}

Factual incorrectness can often be categorised into commonly occurring types such as the following: 
\uls
\li \textbf{Misrepresentation}: This involves presenting information in a way that is misleading or that gives a false impression. This could be done by exaggerating certain aspects, understating others, or twisting facts to fit a particular narrative. An example is providing false information on a local authority's response to a disease outbreak within an area.

\li \textbf{Inaccurate Quantities or Measurements}: Factual incorrectness can occur when precise quantities, measurements, or statistics are misrepresented, whether through error or intent. An example is false information on the number of people hospitalised for a disease outbreak.

\li \textbf{False Attribution}: Incorrectly attributing a statement, idea, or action to a person or group is another form of factual incorrectness. An example is falsely claiming that the World Health Organization (WHO) has confirmed an epidemic status to a disease within a locality.

\li \textbf{Fabrication}: Making up data, sources, or events is a severe form of factual incorrectness. This involves creating `facts' that have no basis in reality, e.g., the outbreak being linked to a genetically modified strain and the story of how it escaped from a research lab.


\ule

In our work, we plan to annotate a dataset of the common types of  factual incorrectness (the gold-standard ground-truth data), and also explore ways to generate the data automatically with LLMs via suitable prompts (the silver-standard ground-truth data). Again, similar to the binary classification approach, we also plan to investigate the combination of fine-tuned transformer based approach and in-context learning to address this task.


\subsubsection{Extracting or summarising the misinformation}
Instead of predicting if a text segment contains misinformation and the type of misinformation it contains, in this work we plan to also identify the span of text (e.g., at sentence or sub-sentence level) that contains misinformation. This would particularly be advantageous for relatively large documents where the reader needs to spend less effort in identifying the misinformation from the context.

This would require training a sequence labeling approach \cite{wang2020adaptive}, which can be fine-tuned on both gold-standard (manually annotated) and silver-standard (LLM-generated) datasets.

\subsubsection{Novel Ideas to Explore in WP-1} \label{ss:wp1}

To model the specific task of misinformation detection, we plan to investigate two novel ideas - i) adaptive in-context learning, and ii) an ensemble of in-context learning with that of supervised learning.

\para{Adaptive In-Context Learning (Adaptive ICL)}

We first provide a brief technical introduction to In-Context Learning (ICL) before describing the idea on Adaptive ICL.

In-context learning (ICL), unlike supervised learning, does not involve training a set of parameters $\theta$ on labeled examples; rather, the posteriors are now a function of the input claim, the decoder parameters of a pre-trained large language model (LLM), given prompt and optionally a set of $k$ input examples (commonly called $k$-shot examples). Formally,
\begin{equation}
P(y=1|\vec{x}) = f(\vec{x}, \mathcal{P}_k(\vec{x}); \phi_{\text{LLM}}),
\label{eq:icl}
\end{equation}
where, different from a supervised setup, the function $f$ does not have a parameterized representation that can be learned using a training set with gradient descent. The function itself depends on the pre-trained parameters $\phi_{\text{LLM}}$ of an LLM, the current inputs for which a label is to be predicted, and a prompt comprising a set of $k$ text units denoted by $\mathcal{P}_k(\vec{x})$.
Since the decoder of an LLM generates a sequence of words of the form of $w_1,\ldots,w_M$ ($M$ being the maximum length of a sequence), the class posterior likelihoods are computed by mapping the $c$ possible classes into $c$ different equivalent sets of words \cite{hu2021knowledgeable}, say $V(y)$, where $y \in \mathbb{Z}_c$. Specifically, in the context of our (binary) misinformation detection problem, $c=2$ (i.e., $y \in \{0, 1\}$), and we define the two sets as: $V(0) = \{\text{`false'}, \text{`negative'}\}$, and $V(1) = \{\text{`true'}, \text{`positive'}\}$. 

The idea of adaptive ICL centres around choosing the context $\mathcal{P}_k(\vec{x})$ in a data-driven manner, i.e., making $k$ a function of the data (current instance $\vec{x}$) itself. This is somewhat analogous to choosing a different value of $k$ for a $k$-NN based non-parametric modeling. The motivation is that classifying some instances would be more difficult than others, in which cases they are potentially to be benefited from a larger value of $k$ (more context). On the other hand, for relatively easy data instances using too much context may be detrimental for effective prediction.

Generally speaking, given a training set of points, the idea would hence be to train a classifier that predicts an optimal value of $k$ from among a number of choices. Specifically speaking, for a given $k_{max}$ (a parameter), during the training phase we would try substituting progressively increasing values of $k$ in Equation \ref{eq:icl}, and choose the one where the prediction matches the true label. This will yield the minimal context (smallest $k$, where $k \leq k_{max}$) for effective classification, and will serve as a label for an auxiliary task of context size prediction. More specifically, we propose to train a parametric classifier (e.g., logistic regression or, more generally, a feed-forward network with multiple layers) to `learn' this optimal value of context size ($k$) for a given $\vec{x}$, i.e.,
$\theta(\vec{x}) \mapsto \text{argmin}_{k\leq k_{max}} \mathbb{I}(f(\vec{x}, \mathcal{P}_k(\vec{x}))= y(\vec{x}))$.
During inference time, we make predictions for the downstream task (in this case that of misinformation detection) with
\begin{equation}
P(y=1|\vec{x}) = f(\vec{x}, \mathcal{P}_{\theta(\vec{x})}(\vec{x}); \phi_{\text{LLM}}),
\label{eq:icl}
\end{equation}
where $\theta(\vec{x})$ is the context size predicted with the classifier function $\theta$ learned during the training phase.

\para{Ensemble of Supervised Learning and ICL}

The next novel idea that we intend to investigate is a combination of a parametric approach $P(y|\vec{x}) = g(\vec{x}, y(\vec{x}; \zeta)$ (parameters $\zeta$ learned by a loss function such as cross-entropy), with ICL (Equation \ref{eq:icl}), which essentially is a non-parametric approach (parameters $\phi$ for the LLM are frozen).





\subsection{WP-2: Explainable In-Context Learning}

In this work package, we plan to explain the working mechanism of In-Context Learning (ICL). We first start with a brief introduction to explainable AI, following which we describe our proposed idea of explainable ICL.

\subsubsection{A Brief Introduction to Explainable AI}
Given a data instance $\vec{x}$ and a parameterized (trained) model $\theta: \vec{x} \mapsto y$, existing models of per-instance explanations (e.g. LIME \cite{Ribeiro}, L2X \cite{L2X} or Shap \cite{SHAP}) first sample other similar data instances, $\vec{z} \in N(\vec{x})$, from its neighborhood and then learns a \emph{local view} of the black-box model $\theta$ by making use of the predictions on these \emph{local} instances.
The instance-wise explanation objective is to make the local model $\theta_{\vec{x}}$ \emph{closely approximate} the global model $\theta$, the objective being to minimize a loss of the form
\begin{equation}
\mathcal{L}(\vec{x},\theta; \phi) = \!\!\!\!\!\!\sum_{\vec{z} \in N(\vec{x})}
\!\!\!(\theta(\vec{z}) - \phi\cdot\vec{z})^2,\,\,
N(\vec{x})= \{\vec{x}\odot\vec{u}: \vec{u}\sim \{0,1\}^d\} \label{eq:instance_exp},
\end{equation}
where $\phi\cdot\vec{z}$ is a parameterized linear representation of the local function $\theta_{\vec{x}}$. The neighborhood function is approximated by selecting arbitrary subsets of features of the current instance $\vec{x}$ (of the form $\vec{x}\odot \vec{u}$, where $\vec{u}$ is a random bit vector of size $d$, $d$ being the dimensionality of the input). A set of data instances with diverse explanation weights (e.g., as computed with an approximate set cover in \cite{Ribeiro}) may then constitute a global explanation unit for a model.

\subsection{Explainable In-Context Learning}

There are three different levels at which the attention weights in Explainable ICL can be inferred - one at the level of the current instance $\vec{x}$ (which is similar to the existing work on per-instance explanations, e.g. LIME etc.), another at the level of the prompt string (few-shot examples) $\mathcal{P}_k(\vec{x})$, and yet another at the level of the output verbaliser terms (i.e., terms which are used to define the classes in the downstream task).

Recall from Equation \ref{eq:icl} of Section \ref{ss:wp1} that the black-box model in ICL $f$ is a function of the LLM (frozen) parameters $\phi_{\text{LLM}}$, and being a non-parametric approach, that of the input instance $\vec{x}$ along with the its context (prompt) $\mathcal{P}_k(\vec{x})$. This means that explanations only at the level of features (as obtained in LIME, SHAP etc. in terms of feature attribution) is not adequate. There are other data elements on which feature attribution can be carried out.

More specifically, the effect of words in the context (prompt) of an input, i.e., $\mathcal{P}_k(\vec{x})$, can be investigated. An attention weight inferred over a prompt string could then throw insights on how an LLM $\phi_{\text{LLM}}$ leverages contextual information. For instance, an ICL model that puts more emphasis on terms from the $k$-shot examples that are semantically related to the downstream task could potentially be considered more trustworthy than a model which emphasises on semantically unrelated terms.

As a concrete example, consider a sentence on the topic of a disease outbreak in a locality, which is to be classified as misinformation or not by an ICL-based classifier. The classifier takes as input the current sentence and two 1-shot examples (one from each class). Let us suppose that we infer the attention weights (more details of which follows in the next section) of the examples. It can be argued that a model LLM
$\phi_{\text{LLM}}$
which puts emphasis on words such as
`disease' and `epidemic' is potentially more trustworthy than another model
LLM $\phi'_{\text{LLM}}$
which emphasises instance-specific terms, such as the name of the locality etc.


\subsection{Inferring the Attention Weights in Explainable ICL}

Formally speaking, the attention weights over the input $\vec{x}$, and the prompt $\mathcal{P}_k(\vec{x})$ can be derived by defining similar neighborhoods (Equation \ref{eq:instance_exp}) around them. In particular, the two neighborhoods can then be used to learn two auxiliary per-instance explanation models by applying a method similar to Equation \ref{eq:instance_exp}.
\begin{equation}
N(\vec{x})= \{\vec{x}\odot\vec{u}: \vec{u}\sim \{0,1\}^d\},\,\,\,
N(\mathcal{P}_k(\vec{x}))= \{\mathcal{P}_k(\vec{x})\odot\vec{u}: \vec{u}\sim \{0,1\}^d\}.
\end{equation}

A similar approach can then be adapted for the `verbaliser to output class mapper' to learn the attention weights for the terms defining the output classes, or a more direct approach of counter-factual based explanations \cite{verma2022counterfactual} can also be applied.


\section{WP-3: Fair In-Context Learning}

While previous work in AI has attempted to mitigate biases from supervised models \cite{cyberbullying,equality_opportunity,discriminationPrevention,knn_discriminationpreven,discrimination_DM}, in this work-package of the proposed project we plan to investigate bias mitigate for In-Context Learning (ICL). This is an important problem to investigate because ICL has proven to be more effective than their supervised counterparts (likely due to the advantages of pre-training on massive volumes of text), and it is likely that ICL will likely be used in combination with (or even as a substitute for) supervised learning in near future.

\subsection{Introduction to Fair AI}

The ubiquitous use of data-driven (deep) learning has led to risks of these models learning their own characteristic abstractions of the data, often eventually manifested as stereotype societal biases in their predictions \cite{cyberbullying,equality_opportunity,discriminationPrevention,knn_discriminationpreven,discrimination_DM}, examples of which may include predicting more frequently that women are weaker as compared to men \cite{kiritchenko-mohammad-2018-examining}, or that African Americans are more likely to commit crimes than Caucasians \cite{propublica}.
The main reason why such biases manifest themselves into deep neural models is due to the data-only training mode (not involving any manually engineered features), which means that there is
a smaller degree of control on how the task-specific data abstractions are constructed via the model parameters (e.g., for a feature-based model, it is possible to leave out a certain set of features to a model, e.g., the race of a person for recidivism prediction \cite{propublica,adDelivery}).


\subsection{Proposed Methodology}

Existing bias mitigation methods can be classified into three general categories as follows: (i) \textbf{Pre-processing methods}, which modify the training dataset before feeding it to the DL model; these approaches modify the prior distributions of the attribute (metadata) variables (e.g., age, gender etc.), or more generally, perform specific transformations on the data with an aim to reduce disparity of the class priors in the training data \cite{Kamiran2011DataPT,discr_preven,bolukbasi:2016,gonen-goldberg-2019,liang-etal-2020-towards}; (ii) \textbf{In-process methods}, which employ a multi-task learning with a bias-specific objective added to the primary task objective \cite{inprocessing,Beutel2017DataDA,DBLP:conf/emnlp/CoavouxNC18,Sen2020TowardsSR, few_shot_fair} or an adversarial loss component \cite{blind-eye,adversarial,DBLP:conf/sigir/RekabsazKS21}; (iii) \textbf{Post-processing methods}, which modify the final decisions of the classifiers by transforming model outputs to improve prediction fairness \cite{post-processing}
(also see \cite{Caton2020FairnessIM} for an overview).

In this project, we will explore a combination of pre-processing, in-processing and post-processing approaches for bias mitigation. The in-process method will investigate the use of LLM-generated prompts as contexts to modify the output of ICL (recall that ICL predictions are a function of both the input $\vec{x}$ and the context $\mathcal{P}_k(\vec{x})$). Specifically, we plan to use few shot examples of stereotyped and anti-stereotyped predictions as contexts to an LLM for ICL, e.g., to predict if `girls love fairytales' is stereotype one could use related examples, such as `boys do not cry' (labelled stereotype) and `boys are emotionally weak' (labelled anti-stereotype) as contexts to an LLM to mitigate the problems of stereotype predictions.


    
 








\section{EPSRC Criteria Checkbox} \label{sec:checkbox}

\para{Timely given current trends, and quality and importance of the proposed research}
The proposed research is timely because the in-context learning (ICL) with LLMs is a relatively new concept \cite{peters-etal-2018-deep, radford2019language,liu2021gpt,brown2020language}. Although it has been established as new state-of-the-art for a number of different tasks, ranging from classification to ranking, there are a large number of research questions that are not yet addressed in a systematic manner.
Investigating \textbf{adaptive ICL} (WP-1) can potentially improve the effectiveness of ICL-based predictions thus further advancing the field.

\para{Potential to advance current understanding}

Exploring the \textbf{explainability of ICL} models (WP-2) would add further insights to our understanding of these models and potentially make these models more trustworthy by aligning their abstractions of the data with those of humans. This will help deploying such models in critical applications such as medical diagnosis, legal judgment prediction etc. 

\para{Generates new knowledge, thinking or discovery}

The work conducted towards addressing the research questions on adaptive, explainable and fair ICL would throw insights on how to effectively apply the potential of LLMs on a range of different AI tasks.

\para{Direct or indirect benefits}
The work proposed in the project will not only provide a direct benefit of developing \textbf{effective AI} models for a range of different NLP tasks (e.g., classification) but will also potentially have a societal impact in developing \textbf{responsible AI}, i.e., trustworthy and fair predictive models.
A specific application of misinformation detection (in the age of generative LLMs, where it is easy to generate fabricated information) has an important societal benefit in the form of 
fostering communal harmony and ensuring a healthier societal structure.

